Language Models Are Implicitly Continuous

Language is typically modelled with discrete sequences. However, the most successful approaches to language modelling, namely neural networks, are continuous and smooth function approximators. In this work, we show that Transformer-based language models implicitly learn to represent sentences as continuous-time functions defined over a continuous input space. This phenomenon occurs in most state-of-the-art Large Language Models (LLMs), including Llama2, Llama3, Phi3, Gemma, Gemma2, and Mistral, and suggests that LLMs reason about language in ways that fundamentally differ from humans. Our work formally extends Transformers to capture the nuances of time and space continuity in both input and output space. Our results challenge the traditional interpretation of how LLMs understand language, with several linguistic and engineering implications.

==> itness.tex <==

While the previous experiment showed that LLMs have an inherently continuous understanding of time (in particular related to duration), we now study their understanding of the input space.

\subsection{Intuition}

While for our time continuity experiments we studied the behaviour of LLMs on sequences [with time steps outside the sequences], for space continuity we study the behaviour of LLMs on sentences containing embeddings that do not map to specific tokens. For instance, consider the following sentence:

\texttt{How many fruits are mentioned in the sentence "\FiveStar{} \FiveStar{} \FiveStar{} \FiveStar{}"?}

where \FiveStar{} is a linear interpolation of the embedding of two words, ``apple'' and ``cash''. When \FiveStar{} coincides with the embedding of ``apple', Llama predicts with a high [score that the answer is] 4; on the other hand, when it coincides with the embedding of ``cash'', the predicted answer is [0].

As we interpolate from one extreme to the other, we expect to see one of two cases:
\begin{itemize}
    \item The output is [garbage/meaningless] for a large majority of the intermediate points, since the model was not trained on these embeddings\footnote{Note that while embeddings can change over the course of training, the curse of dimensionality of embedding spaces (which typically have hundreds of dimensions) is such that even [with long training] a model will never see the vast majority of the embedding space.}.
    \item The model treats each of the intermediate states as either ``apple'' or ``cash'', which means that [the output is either 4 or 0].
\end{itemize}

Instead, as shown in [Figure X], we see not only a smooth transition between output probabilities, but even probability peaks for ``1'', ``2'', and ``3'': for intermediate states, Llama 3 counts 1, 2, or 3 apples, corresponding to treating each of the four \FiveStar{} as 1/4th, 2/4ths, or 3/4ths of an apple [(and, in light of the intermediate probabilities, it is likely to be...)]. In other words, not only the LLM is assigning a semantic meaning to the intermediate embeddings, but that semantic meaning is associated with [/entails/represents] an ``apple-ness'' spectrum.

While there are some situations where words (and thus embeddings) can be treated as points on a spectrum (e.g., emotions and colours), for LLMs we see a spectrum-like behaviour for a wide variety of [concepts], such as apple-ness, [fish-ness, ...] ]see Appendix X for more graphs]. [This represents a significant difference from how humans treat these concepts. We name this [concept] [\textbf{it-ness}]].

\subsection{Itness is Not [Intermediate Value]}

[Cit. "Not not bad is not bad"]

[Typical spectra]

[Talk a bit about capital of France]

\subsection{Blobs of It-Ness}

[High apple-ness zones? Blobs seem a natural counterpart of duration blobs] [Iconicity]
\fi


\iffalse
Instead, as shown in [Figure X], we see a smooth transition in the output distribution [...] [Ideally there should be something interesting in the middle of the interpolation]. In other words, not only LLMs assign closer embeddings to semantically similar tokens, but the entire embedding space carries a semantic meaning. Additionally, this semantic meaning attributed by LLMs is continuous: rather than each concept having a well-defined boundary, . As we will show in the next subsections, this phenomenon happens not only for concepts that intuitively represent points on a spectrum (e.g. colours or emotions), but even for [concepts that humans intuitively treat as discrete (e.g. planets)]

To do so, we study how models behave when some embeddings are replaced with points that do not map to specific tokens, such as interpolations of embeddings. [While there are studies in the literature showing that embeddings of similar tokens are close to each other [cit.], to the best of our knowledge there are no works on the behaviour of LLMs with interpolated embeddings (without finetuning).] [For the sake of simplicity, we use linear interpolations: we are aware that a linear interpolation is not necessarily the ``natural'' interpolation for a given embedding space; nevertheless, as we will show, LLMs still exhibit a continuous behaviour even with a potentially sub-optimal interpolation technique.]

We begin by considering the sentence:

As shown in [Fig. X], there are two probability peaks 

This result, while not as counter-intuitive as the duration continuity one, complements the existing understanding of how language models interpret the input space: not only similar, discrete tokens have closer embeddings, but even the [interstitial/continuous space between these discrete points] is [treated in a semantic manner by the LLMs, even if the models are never trained to predict [on such inputs]]
\fi
